RRSR:Reciprocal Reference-based Image Super-Resolution with Progressive Feature Alignment and Selection

Reference-based image super-resolution (RefSR) is a promising SR branch and has shown great potential in overcoming the limitations of single image super-resolution. While previous state-of-the-art RefSR methods mainly focus on improving the efficacy and robustness of reference feature transfer, it is generally overlooked that a well reconstructed SR image should enable better SR reconstruction for its similar LR images when it is referred to as. Therefore, in this work, we propose a reciprocal learning framework that can appropriately leverage such a fact to reinforce the learning of a RefSR network. Besides, we deliberately design a progressive feature alignment and selection module for further improving the RefSR task. The newly proposed module aligns reference-input images at multi-scale feature spaces and performs reference-aware feature selection in a progressive manner, thus more precise reference features can be transferred into the input features and the network capability is enhanced. Our reciprocal learning paradigm is model-agnostic and it can be applied to arbitrary RefSR models. We empirically show that multiple recent state-of-the-art RefSR models can be consistently improved with our reciprocal learning paradigm. Furthermore, our proposed model together with the reciprocal learning strategy sets new state-of-the-art performances on multiple benchmarks.

==> sections/charts.tex <==



















% \begin{figure}[t]
% \begin{minipage}[c]{0.6\linewidth}
% \centering
% \includegraphics[width=6.7cm]{figures/rab.pdf}
% \end{minipage}
% \begin{minipage}[c]{0.4\linewidth}
% \caption{Reference-aware block in CIFT. We extract reference-aware information from \textit{input features} and \textit{aligned reference features}. \textit{Input features} and \textit{aligned reference features} are processed by the dynamically-assembled filters, which are conditioned on reference-aware information. It exploits reference-aware information so as to adaptively fuse them. After that, the fused features feature channels is further refine. $k$ is the number of learnable template filters.}
% \label{fig:mask_heads}
% \end{minipage}
% \end{figure}



% \begin{table}[t]
% \caption{Ablation study on TODO.}
% \label{table:ablation_eft}
% \begin{center}
% \resizebox{0.85\textwidth}{!}{
% \begin{tabular}{l|c|c}
% \hline
% Model &RTRR &PSNR $\uparrow$ / SSIM$\uparrow$ \\
% \hline
% C2-matching$^*$      &            & $28.40$ / $0.846$ \\ 
% C2-matching$^*$+RTRR & \checkmark & $28.64$ / $0.853$ \\
% MASA$^*$             &            & $27.47$ / $0.815$ \\ 
% MASA$^*$+RTRR        & \checkmark & $27.58$ / $0.818$ \\
% TTSR$^*$             &            & $27.03$ / $0.800$ \\ 
% TTSR$^*$+RTRR        & \checkmark & $27.17$ / $0.804$ \\
% \hline
% \end{tabular}
% }
% \end{center}
% \end{table}


% \begin{table}[t]
% \caption{Ablation study on TODO.}
% \label{table:ablation_eft}
% \begin{center}
% \resizebox{0.85\textwidth}{!}{
% \begin{tabular}{l|c|c|c|c}
% \hline
% Model &PFA &RAS &RTRR &PSNR $\uparrow$ / SSIM$\uparrow$ \\
% \hline
% Baseline(C2-matching$^*$) &            &            &            & $28.40$ / $0.846$ \\
% Baseline+PFA            & \checkmark &            &            & $28.63$ / $0.851$ \\
% Baseline+PFA+RAS        & \checkmark & \checkmark &            & $28.70$ / $0.853$ \\
% Baseline+PFA+RAS+RTRR   & \checkmark & \checkmark & \checkmark & $28.83$ / $0.856$ \\
% \hline
% \end{tabular}
% }
% \end{center}
% \end{table}




